AST-T5: Structure-Aware Pretraining for Code Generation and Understanding

Large language models (LLMs) have made significant advancements in code-related tasks, yet many LLMs treat code as simple sequences, neglecting its structured nature. We introduce AST-T5, a novel pretraining paradigm that leverages the Abstract Syntax Tree (AST) for enhanced code generation, transpilation, and understanding. Using dynamic programming, our AST-Aware Segmentation retains code structure, while our AST-Aware Span Corruption objective equips the model to reconstruct various code structures. Unlike other models, AST-T5 avoids intricate program analyses or architectural changes, so it integrates seamlessly with any encoder-decoder Transformer. Evaluations show that AST-T5 consistently outperforms similar-sized LMs across various code-related tasks. Structure-awareness makes AST-T5 particularly powerful in code-to-code tasks, surpassing CodeT5 by 2 points in exact match score for the Bugs2Fix task and by 3 points in exact match score for Java-C# Transpilation in CodeXGLUE. Our code and model are publicly available at https://github.com/gonglinyuan/ast_t5.

==> figures/humaneval.tex <==
\begin{figure}[t]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[]{figures/fig_humaneval.pdf}}
\caption{Visualization of \model's performance on HumanEval compared to models exceeding 230M parameters and thus not detailed in Table 2. Each point on the scatter plot represents a model. The x-axis shows the parameter count in log-scale, while the y-axis shows the Pass@1 rate on HumanEval in log-scale. Model open-source status is color-coded: \textcolor{blue}{\textbf{blue}} for open-source and \textcolor{red}{\textbf{red}} for proprietary.}\label{fig:humaneval}
\end{center}
\vskip -0.2in
\end{figure}


==> figures/mbpp.tex <==
\begin{figure}[t]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[]{figures/fig_mbpp.pdf}}
\caption{Visualization of \model's performance on MBPP compared to other models. Each point on the scatter plot represents a model.}\label{fig:mbpp}
\end{center}
\vskip -0.2in
\end{figure}

